Disparate Impact on Group Accuracy of Linearization for Private Inference

Ensuring privacy-preserving inference on cryptographically secure data is a well-known computational challenge. To alleviate the bottleneck of costly cryptographic computations in non-linear activations, recent methods have suggested linearizing a targeted portion of these activations in neural networks. This technique results in significantly reduced runtimes with often negligible impacts on accuracy. In this paper, we demonstrate that such computational benefits may lead to increased fairness costs. Specifically, we find that reducing the number of ReLU activations disproportionately decreases the accuracy for minority groups compared to majority groups. To explain these observations, we provide a mathematical interpretation under restricted assumptions about the nature of the decision boundary, while also showing the prevalence of this problem across widely used datasets and architectures. Finally, we show how a simple procedure altering the fine-tuning step for linearized models can serve as an effective mitigation strategy.

==> tex_files/acknowledgements.tex <==
This research is partly funded by NSF grants SaTC-2345483, RI-2334936, and CAREER-2401285. F. Fioretto is also supported by a Google Research Scholar Award and an Amazon Research Award. The views and conclusions of this work are those of the authors only.

==> tex_files/contributions.tex <==
This paper makes the following contributions:
\textbf{(1)} We observe, for the first time, a Matthew's effect on accuracy reduction caused by the targeted linearization process adopted to reduce the number of \gls*{relu} functions in private inference methods. 
Further, we show that such disparity is exacerbated as the number of approximated \gls*{relu} functions grows.
\textbf{(2)} We present a mathematical interpretation of this phenomenon, which relates these disparity effects with the approximation capabilities of \gls*{relu} functions  
when assumptions on the space of the decision boundaries can be made.
\textbf{(3)} We show that the effect of \gls*{relu} reduction on fairness is vastly present for commonly deployed algorithms and models when trained on unbalanced datasets. 
\textbf{(4)} Finally, we propose a simple yet effective mitigation strategy that can be applied to any framework for \gls*{relu} reduction, during the training or fine-tuning phase, showing favorable results in terms of fairness.
